Exploring Pose-Based Anomaly Detection for Retail Security: A Real-World Shoplifting Dataset and Benchmark

Shoplifting poses a significant challenge for retailers, resulting in billions of dollars in annual losses. Traditional security measures often fall short, highlighting the need for intelligent solutions capable of detecting shoplifting behaviors in real time. This paper frames shoplifting detection as an anomaly detection problem, focusing on the identification of deviations from typical shopping patterns. We introduce PoseLift, a privacy-preserving dataset specifically designed for shoplifting detection, addressing challenges such as data scarcity, privacy concerns, and model biases. PoseLift is built in collaboration with a retail store and contains anonymized human pose data from real-world scenarios. By preserving essential behavioral information while anonymizing identities, PoseLift balances privacy and utility. We benchmark state-of-the-art pose-based anomaly detection models on this dataset, evaluating performance using a comprehensive set of metrics. Our results demonstrate that pose-based approaches achieve high detection accuracy while effectively addressing privacy and bias concerns inherent in traditional methods. As one of the first datasets capturing real-world shoplifting behaviors, PoseLift offers researchers a valuable tool to advance computer vision ethically and will be publicly available to foster innovation and collaboration. The dataset is available at https://github.com/TeCSAR-UNCC/PoseLift.

==> Sections/Secion_1_introduction_old.tex <==
\section{Introduction}
\label{sec:intro}

Shoplifting is an ongoing concern in modern society, impacting businesses, communities, and the economy at large. It is a complex and persistent issue for retailers, law enforcement, and other stakeholders involved in retail security \cite{ansari2022expert}. As an illegal activity that often goes undetected, it results in significant financial losses for businesses and escalates operational costs. In the United States, the scale of these losses has become increasingly alarming, with retail theft rising yearly.
In 2022, retailers suffered \$112.1\ billion in lost gross revenue; in 2023 alone, stores lost an estimated \$121.1\ billion to retail theft. Projections indicate that shoplifting could exceed \$143\ billion by 2025, as illustrated in \cref {fig:shoplifting_statistics} \cite {shoplifting_capitalone2024}. 

\begin{figure}[htp]
  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[trim=0pt 0pt 0pt 0pt, clip, width=3.4 in]{Figures/shoplifting_statistics.png}
   %left/bottom/right/top
   \caption{Retail sales revenue lost to shoplifting in the USA (in billions), with losses reaching nearly \$122\ billion in 2023 and projected to surpass \$143\ billion by 2025.\cite{shoplifting_capitalone2024}}
   \label{fig:shoplifting_statistics}
\end{figure}

Despite the growing financial impact and losses of shoplifting in the retail sector, traditional security measures have proven insufficient, with retailers managing to catch shoplifters in only about 2\% of cases \cite {shoplifting_capitalone2024}.

In light of these challenges, innovative solutions are being explored to improve real-time monitoring and detection capabilities. One promising approach is the use of AI-powered systems, which have seen increasing deployment in a variety of domains \cite{zibaeirad2024vulnllmeval, doroudian2022study, abshari2024llm}. One such area where AI has shown significant promise is in video surveillance \cite{pazho2023ancilia}. With the growing deployment of surveillance cameras in public spaces to enhance safety, vast amounts of video data are generated, yet security personnel cannot process this data in real-time. This has led to a growing demand for automated systems capable of detecting shoplifting incidents \cite {arroyo2015expert, muneer2023shoplifting}. AI-powered detection techniques enable real-time analysis of video footage to identify theft, with applications in retail stores, marketplaces, and shopping malls. By integrating these systems with existing security infrastructure, theft prevention can be more effective. The system provides real-time alerts for security personnel and helps store managers identify high-risk areas and peak shoplifting times, offering valuable insights to improve security strategies \cite {kirichenko2022detection}. 


The problem of shoplifting detection is particularly challenging due to several inherent factors. A key issue is the scarcity of labeled data, as shoplifting events are both rare and unpredictable, making them difficult to capture in real-world environments. The infrequency of such incidents, combined with the logistical challenges of obtaining annotated examples, severely limits the applicability of supervised machine learning models, which depend on extensive labeled datasets. Additionally, the diverse and unpredictable nature of shoplifting behavior complicates detection. Shoplifters employ a wide range of strategies, from subtle concealment to overt theft, that do not conform to fixed patterns or predefined categories. Another major difficulty arises from the contextual variability of shoplifting, where behaviors can differ significantly across retail environments depending on store layouts, the types of products sold, and customer dynamics.

Unsupervised anomaly detection offers a promising approach to address these challenges. This method involves identifying deviations from typical patterns of behavior, making it well-suited for scenarios where anomalous events are rare or unpredictable. By learning the characteristics of normal shopping activities, unsupervised models do not require labeled instances of shoplifting for training, effectively overcoming the data scarcity issue. Furthermore, the flexibility of anomaly detection methods allows them to adapt to diverse and unpredictable behaviors, as any deviation from normal activity can be flagged as anomalous. Finally, the open-set nature of unsupervised anomaly detection enables adaptability across different retail contexts, accommodating variations in shoplifting behavior and environmental factors. This adaptability is crucial for designing scalable and generalizable solutions for retail security.

While unsupervised anomaly detection solves many challenges in shoplifting detection, issues such as privacy and bias remain unresolved. Privacy is a significant concern, as using raw video data in retail environments can compromise the confidentiality of individuals in public spaces. Additionally, detection models may unintentionally introduce bias by focusing on physical attributes such as gender, race, or clothing style, potentially leading to unfair and unethical outcomes. A practical solution is to shift from raw pixel-based data to higher-level representations such as human pose, which abstracts personal features while retaining essential information for identifying anomalous behavior. This approach addresses privacy concerns by anonymizing data and reduces bias by ensuring that models prioritize actions over appearances.

The scarcity of data also leads to a lack of robust, real-world datasets. To address this issue, researchers have often resorted to combining data from multiple online sources or staging shoplifting scenarios with hired actors. While these approaches provide some utility, they fail to accurately represent the complexities and nuances of real-world shoplifting behavior. Specifically, they overlook the contextual and environmental factors unique to individual retail stores, which are critical for developing effective and context-aware detection systems. This disconnect between artificially generated datasets and real-world scenarios limits the practical applicability of existing research and highlights the need for datasets that reflect authentic shoplifting behaviors in diverse retail settings.


Building on the challenges discussed, this paper introduces a novel perspective on shoplifting detection by framing it as an unsupervised anomaly detection problem and leveraging pose-based data to address biases and privacy concerns. To achieve this, we present PoseLift, a real-world benchmark dataset that captures authentic shoplifting scenarios recorded in a local retail store. Unlike previous datasets, which rely on staged scenarios with actors, PoseLift consists entirely of real-world incidents, providing a more realistic representation of the problem. In line with privacy considerations, the dataset includes only anonymized data such as bounding boxes, tracking IDs, and human poses, ensuring that no personally identifiable information is used.

To evaluate the effectiveness of this approach, we conduct comprehensive experiments treating shoplifting detection as an unsupervised anomaly detection task. Using state-of-the-art pose-based anomaly detection models, we benchmark their performance on PoseLift using a comprehensive set of metrics, including Area Under The Receiver Operating Characteristic Curve (AUC-ROC), Area Under the Precision-Recall Curve (AUC-PR), and Equal Error Rate (EER), analyzing their potential benefits for addressing the challenges of shoplifting detection. This study provides insights into the utility of pose-based unsupervised methods and establishes a foundation for future research in privacy-preserving retail security. Our dataset will be publicity available to support research and algorithmic development aimed at enhancing safety protocols and improving shoplifting detection systems. The main contribution of this study can be ordered as follows: 


% By utilizing pose-based anomaly detection algorithms, the biases of traditional pixel-based methods can also be reduced \cite {noghre2024pheva, alinezhad2023understanding, noghre2024exploratory}. To support this approach, we introduce a privacy-preserving shoplifting detection dataset, which only includes de-identified human annotations such as bounding boxes, tracking IDs, and human poses. Our Developed dataset provides a benchmark for pose-based shoplifting detection algorithms. 

% While previous studies have proposed several datasets and methods for shoplifting detection, many are based on simulated shoplifting scenarios and rely on pixel-based algorithms \cite {ansari2022esar,ansari2023optimized, nazir2023suspicious, kirichenko2022video}. 
% The availability of real-world datasets in this field is limited, as anomalous shoplifting behaviors are both rare and difficult to capture. This limitation is further compounded by the privacy and ethical concerns surrounding the use of real video data for shoplifting detection, making it essential to approach the collection and sharing of such datasets with sensitivity. In response to these challenges, we take a novel approach by treating shoplifting detection as a pose-based anomaly detection task.

% Building on this, we conduct a comprehensive set of experiments to evaluate the effectiveness of our dataset. Not only do we statistically compare our developed dataset with existing ones, but we also benchmark state-of-the-art pose-based anomaly detection algorithms to assess the learnability of the data. These algorithms are evaluated using a comprehensive set of metrics, including Area Under The Receiver Operating Characteristic Curve (AUC-ROC), Area Under the Precision-Recall Curve (AUC-PR), and Equal Error Rate (EER). Our dataset will be publicity available to support research and algorithmic development aimed at enhancing safety protocols and improving shoplifting detection systems. The main contribution of this study can be ordered as follows: 
\begin{itemize}
    \item Framing shoplifting as anomaly detection: We model shoplifting detection as an anomaly detection problem, focusing on identifying atypical behaviors within retail environments. 
    
    \item Development of a privacy-preserving, real-world shoplifting detection dataset: We introduce a real-world privacy-preserving dataset with de-identified annotations for both normal shopping and shoplifting behaviors.

    \item Benchmarking anomaly detection algorithms: We evaluate state-of-the-art pose-based anomaly detection algorithms, including STG-NF \cite{hirschorn2023normalizing}, TSGAD \cite{noghre2024exploratory}, and GEPC \cite{markovitz2020graph}, on the dataset using metrics like AUC-ROC, AUC-PR, and EER, to thoroughly evaluate the dataset.
  
\end{itemize}


% there is still a lack of comprehensive benchmark dataset that is both large-scale and real-world, suitable for model training, and capable of representing a wide range of both shoplifting and normal shopping behaviors.

